Random Matrix Theory Model for Mean Notch Depth of the Diagonally Loaded MVDR Beamformer for a Single Interferer Case

Adaptive beamformers (ABFs) suppress interferers by placing a notch in the beampattern at the interferer direction. This suppres- sion improves detection of a weaker signals in the presence of strong interferers. Hence the notch depth plays a crucial role in determining the adaptive gain obtained from using ABF over conventional beam- forming. This research derives models for the mean notch depth of a diagonally loaded MVDR ABF for a single interferer case. The model describes the mean notch depth as a function of number of snapshots, the number of sensors in the array, the interferer to noise ratio (INR) level, the interferer direction and the diagonal loading level. The derivation uses random matrix theory results on the be- havior of the eigenvectors of sample covariance matrix. The notch depth predicted by the model is shown to be in close agreement with simulation results over a range of INRs and snapshots.

==> defs.tex <==
% New commands / defs
% Text substitute
\newcommand{\ECM}{ECM}
\newcommand{\cin}{2D isotropic noise}
\newcommand{\marpas}{Mar\v{c}enko-Pastur}

% Formatting commands
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\fig}{Fig.~}
\newcommand{\sect}{Sec.~}
\newcommand{\eqn}{Eq.~}

% Math notation related commands
\newcommand{\AN}{\ensuremath{{\bf A}_N}}
\newcommand{\BN}{\ensuremath{{\bf B}_N}}
\newcommand{\X}{\ensuremath{{\bf X}}}
\newcommand{\x}{\ensuremath{{\bf x}}}
\newcommand{\wt}{\ensuremath{{\bf w}}}
\newcommand{\wts}{\ensuremath{\hat{\bf w}}}
\newcommand{\eye}{\ensuremath{{\bf I}}}  % Identity matrix
\newcommand{\dl}{\delta} % Diagonal loading
\newcommand{\wdlmvdr}{\ensuremath{\wt_{MVDR}}}
\newcommand{\rep}{{\bf v}}        % planewave replica
\newcommand{\repmat}{{\bf V}}     % replica matrix
\newcommand{\replook}{\rep_0}
\newcommand{\repint}{\rep_1}
\newcommand{\inv}{^{-1}}
\newcommand{\herm}{^{\rm H}}


% Cov matrices
\newcommand{\ecm}{\bf R}
\newcommand{\scov}{\ensuremath{\hat{\bf R}}}
\newcommand{\ncov}{\ensuremath{\bf{R}_n}}
\newcommand{\nicov}{\ensuremath{\bf{R}_{i+n}}}
\newcommand{\Knn}{\ensuremath{\mathbf{R}_n}}
\newcommand{\sKnn}{\ensuremath{\hat{\mathbf{R}}_n}}
\newcommand{\GNL}{\ensuremath{{\bf \mathcal G}}}
\newcommand{\Wishart}{\ensuremath{{\bf W}(c)}}

% Interferer
\newcommand{\ipow}{\ensuremath{\sigma_1^2}}
\newcommand{\spow}{\ensuremath{\sigma_s^2}}
\newcommand{\taper}{\boldsymbol{T}}
% EVD
\newcommand{\eval}{\ensuremath{\lambda}}
\newcommand{\seval}{\ensuremath{\hat{\lambda}}}
\newcommand{\Eval}{\ensuremath{\boldsymbol{\Lambda}}}
\newcommand{\evec}{\ensuremath{\boldsymbol{u}}}
\newcommand{\Evec}{\ensuremath{\boldsymbol{U}}}
\newcommand{\ensevec}{\boldsymbol{\zeta}}
%PM relatd
\newcommand{\Lmz}{\ensuremath{L_{mz}}}
\newcommand{\WishartUL}{\ensuremath{(1 + \sqrt{c})^2}}
\newcommand{\Threshold}{\ensuremath{(1 + \sqrt{c})}}
\newcommand{\fhat}{\ensuremath{\hat{f}(x)}}

% Array
\newcommand{\sv}[1]{\mathbf{v}(#1)}
\newcommand{\svh}[1]{\mathbf{v}^{H}(#1)}
\newcommand{\tpl}{\frac{2\pi}{\lambda}}


% EDF
\newcommand{\edf}[1]{F^{#1}}
\newcommand{\fMP}{\ensuremath{f_{MP(c)}}} 

% Null broadening
\newcommand{\nullwidth}{\Delta}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "TuladharICASSP14"
%%% End: 

